Overcoming the Spectral Bias of Neural Value Approximation

Value approximation using deep neural networks is at the heart of off-policy deep reinforcement learning, and is often the primary module that provides learning signals to the rest of the algorithm. While multi-layer perceptron networks are universal function approximators, recent works in neural kernel regression suggest the presence of a spectral bias, where fitting high-frequency components of the value function requires exponentially more gradient update steps than the low-frequency ones. In this work, we re-examine off-policy reinforcement learning through the lens of kernel regression and propose to overcome such bias via a composite neural tangent kernel. With just a single line-change, our approach, the Fourier feature networks (FFN) produce state-of-the-art performance on challenging continuous control domains with only a fraction of the compute. Faster convergence and better off-policy stability also make it possible to remove the target network without suffering catastrophic divergences, which further reduces TD}(0)'s estimation bias on a few tasks.

==> Notes/over_estimation.tex <==
\subsection{Over-Estimation and Double Q Learning}

Overestimation is a property of Q-learning where expectation over the maximum of a noisy Q-value consistently induce an overestimation bias~\citep{Thrun1993overestimation}. This happens because the expectation over the max Q,  \(\mathbb E\langle  \max_a Q(s, a) \rangle \) is a \textit{biased} estimator of the quantity \( \max_a  \mathbb E\langle  Q(s, a) \rangle \). This inequality can easily be shown by applying Jensen's inequality~\citep{Jensen1906inequality}, a simple proof we include in Appendix \ref{app:inequality}. Now despite of the systematic nature of this bias, overestimation is expected to gradually vanish given unbounded supply of data~\citep{Thrun1993overestimation}. This indicates that overestimation is in fact resolvable through better function approximation~\citep{Thrun1993overestimation}. Indeed, in \cite{Thrun1993overestimation}, the authors attributes the issue to noise introduced by the neural network function approximator, which now we are able to explain and fully account for, using kernel regression and Gaussian processes view of neural networks~\citep{Neal1996bayesian}

Under this view, the stochasticity of the neural value approximation has two sources. We parameterize the \(Q\) function as \(Q(\theta, x)\), where \(\theta \sim P(\Theta)\) is a distribution of parameters for the network weights. \(x={s_t, a_t, r_t}\) are the collection of transition tuples in a buffer. Given more data, the first source, the \textit{epistemic uncertainty} that results from the lack of data will eventually reduce to zero if the process is deterministic, or the aleatoric uncertainty if the process is stochastic. 

The second source of uncertainty results from the random parameter \(\theta\). Neural value approximation is intrinsically a randomized algorithm where entropy is injected through the random initialization \(\theta_0\). Recent progress in kernel regression methods offers a great description of the statistical property both at initialization \citep{gc} and after each gradient update~\citep{Jacot2018NTK}. Under this view, double Q learning \citealt{Hasselt2010double-Q} and its actor-critic counterpart, twin-delayed deterministic policy gradient (TD3) \cite{Fujimoto2018TD3} are effectively poor person's approximation of a Q-function ensemble~\citep{Lee2020sunrise}. This motivates that a more tightly-bound neural function approximator class can potentially accomplish the same goal, where the only source of uncertainty comes from data. 

==> Overcoming Spectral Bias Neural Value Approximation/Notes/over_estimation.tex <==
\subsection{Over-Estimation and Double Q Learning}

Overestimation is a property of Q-learning where expectation over the maximum of a noisy Q-value consistently induce an overestimation bias~\citep{Thrun1993overestimation}. This happens because the expectation over the max Q,  \(\mathbb E\langle  \max_a Q(s, a) \rangle \) is a \textit{biased} estimator of the quantity \( \max_a  \mathbb E\langle  Q(s, a) \rangle \). This inequality can easily be shown by applying Jensen's inequality~\citep{Jensen1906inequality}, a simple proof we include in Appendix \ref{app:inequality}. Now despite of the systematic nature of this bias, overestimation is expected to gradually vanish given unbounded supply of data~\citep{Thrun1993overestimation}. This indicates that overestimation is in fact resolvable through better function approximation~\citep{Thrun1993overestimation}. Indeed, in \cite{Thrun1993overestimation}, the authors attributes the issue to noise introduced by the neural network function approximator, which now we are able to explain and fully account for, using kernel regression and Gaussian processes view of neural networks~\citep{Neal1996bayesian}

Under this view, the stochasticity of the neural value approximation has two sources. We parameterize the \(Q\) function as \(Q(\theta, x)\), where \(\theta \sim P(\Theta)\) is a distribution of parameters for the network weights. \(x={s_t, a_t, r_t}\) are the collection of transition tuples in a buffer. Given more data, the first source, the \textit{epistemic uncertainty} that results from the lack of data will eventually reduce to zero if the process is deterministic, or the aleatoric uncertainty if the process is stochastic. 

The second source of uncertainty results from the random parameter \(\theta\). Neural value approximation is intrinsically a randomized algorithm where entropy is injected through the random initialization \(\theta_0\). Recent progress in kernel regression methods offers a great description of the statistical property both at initialization \citep{gc} and after each gradient update~\citep{Jacot2018NTK}. Under this view, double Q learning \citealt{Hasselt2010double-Q} and its actor-critic counterpart, twin-delayed deterministic policy gradient (TD3) \cite{Fujimoto2018TD3} are effectively poor person's approximation of a Q-function ensemble~\citep{Lee2020sunrise}. This motivates that a more tightly-bound neural function approximator class can potentially accomplish the same goal, where the only source of uncertainty comes from data. 

==> Overcoming Spectral Bias Neural Value Approximation/figtext/erank.tex <==
\begin{table}[h]
  \caption{Effective rank~\citep{Roy2007effective-rank} of Q value function features learned by RFAC and \TD{} on HalfCheetah, Ant and Humanoid.}
  \label{tbl:erank}
  \centering
  \begin{tabular}{lllll}
    \toprule
          & Half-Cheetah & Ant & Humanoid \\
    \midrule
    RFAC & $2.94 \pm 1.12$ & $2.86 \pm 1.32$ & $2.94 \pm 1.26$ \\
    DDPG  & $1.01 \pm 1.00$ & $1.08\pm 1.07$ & $1.49 \pm 1.22$ \\
    \bottomrule
  \end{tabular}
\end{table}

==> Overcoming Spectral Bias Neural Value Approximation/figtext/rff_abl_bandwidth.tex <==
\begin{figure}[t]
     \centering
          \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/HalfCheetah_diff_b.svg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/Ant_diff_b.svg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/Humanoid_diff_b.svg}
     \end{subfigure}
     \caption{We analyze the performance of RFAC for different values of bandwidth b on HalfCheetah, Ant and Humanoid control tasks.
     While RFAC performs similarly on HalfCheetah and Ant for different values of bandwidth b, its performance varies on Humanoid with different values of b.}
     \label{fig:td3_rff_abl_bandwidth}
\end{figure}

==> Overcoming Spectral Bias Neural Value Approximation/figtext/rff_abl_f_dim.tex <==
\begin{figure}[t]
     \centering
     \includesvg[scale=0.3]{figures/ant_f_dim_4k_vs_400.svg}
     \caption{We analyze the performance of RFAC for state fourier dimensions on Ant. It suffers a significant drop in performance if we decrease its state fourier dimension from $4000$ to $400$.}
     \label{fig:td3_rff_abl_f_dim}
\end{figure}

==> Overcoming Spectral Bias Neural Value Approximation/figtext/rff_abl_indep_rff.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/HalfCheetah_conv.svg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/Ant_conv.svg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/Humanoid_conv.svg}
     \end{subfigure}
     \caption{RFAC's performance drops significantly on HalfCheetah, Ant, and Humanoid if we take Random Fourier Features independently per dimension via 1d convolution and then concatenate them.}
     \label{fig:td3_rff_indep_rff}
\end{figure}

==> Overcoming Spectral Bias Neural Value Approximation/figtext/rff_comp.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/HalfCheetah_comp.svg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/Ant_comp.svg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/Humanoid_comp.svg}
     \end{subfigure}
     \caption{We compare RFAC with \TD{} and other baselines on HalfCheetah, Ant and Humanoid control tasks. It improves over \TD{} and either matches or outperforms \TD-dense on all the tasks. \TD-deep improves over \TD{} and performs similar to RFAC and \TD-dense on HalfCheetah. On Ant and Humanoid, it performs similar to \TD{} implying that overparameterization doesn't always help.}
     \label{fig:td3_rff_comp}
\end{figure}

==> Overcoming Spectral Bias Neural Value Approximation/figtext/rff_dmc.tex <==
\begin{figure}[h]
     \centering
     \includesvg[scale=0.3]{figures/Hopper.svg}
     \caption{DeepMind Control suite domain: Hopper-hop. RFF network has lower variance, and out-performs the vanilla MLP baseline on average.}
     \label{fig:td3_rff_ant}
\end{figure}

==> Overcoming Spectral Bias Neural Value Approximation/figtext/rff_param_comp.tex <==
\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/HalfCheetah_comp_rff.svg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/Ant_comp_rff.svg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/Humanoid_comp_rff.svg}
     \end{subfigure}
     \caption{We compare MLPs with different fourier feature parameterizations on how they perform on continous control tasks. We use \TD{} as the base reinforcement learning algorithm.
    %  We compare RFAC (i.e. \TD{}+RFN) with \TD{}+Siren and \TD{}+RFF-Tancik on HalfCheetah, Ant and Humanoid control tasks. We see that RFAC is able to outperform the other baselines which, in turn, shows that RFN is better suited for high dimensional continuous control tasks when compared to other random fourier feature paramterization.
     }
     \label{fig:rff_param_comp}
\end{figure}

==> Overcoming Spectral Bias Neural Value Approximation/figtext/td3_rff_ant.tex <==
\begin{figure}[h!]
     \centering
     \includesvg[scale=0.3]{figures/Ant_td3_rff.svg}
     \caption{RFF network applied to state-of-the-art TD3 algorithm on Ant. Showing significant performance gain, and a new state-of-the-art result.}
     \label{fig:td3_rff_ant}
\end{figure}

==> Overcoming Spectral Bias Neural Value Approximation/figtext/toy_mdp_decription.tex <==
\begin{figure}[t]
     \centering
     \includegraphics[width=\textwidth]{figures/toy_mdp_detail.pdf}
     \caption{Description of a toy MDP with $\gS = [0,1)$, $\gA = \{0,1\}$, $\gamma = 0.9$ and reward function $r(s,a)=s$. (a) describes its forward dynamics, (b) describes the ground truth Q function, (c) denotes the MLP fit to the Q function with fitted Q iteration (FQI)~\citep{fqi} after $200$ epochs and (d) denotes the same after $8000$ epochs.}
     \label{fig:toy_mdp_description}
\end{figure}

==> figtext/erank.tex <==
\begin{table}[h]
  \caption{Effective rank~\citep{Roy2007effective-rank} of Q value function features learned by RFAC and \TD{} on HalfCheetah, Ant and Humanoid.}
  \label{tbl:erank}
  \centering
  \begin{tabular}{lllll}
    \toprule
          & Half-Cheetah & Ant & Humanoid \\
    \midrule
    RFAC & $2.94 \pm 1.12$ & $2.86 \pm 1.32$ & $2.94 \pm 1.26$ \\
    DDPG  & $1.01 \pm 1.00$ & $1.08\pm 1.07$ & $1.49 \pm 1.22$ \\
    \bottomrule
  \end{tabular}
\end{table}

==> figtext/rff_abl_bandwidth.tex <==
\begin{figure}[t]
     \centering
          \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/HalfCheetah_diff_b.svg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/Ant_diff_b.svg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/Humanoid_diff_b.svg}
     \end{subfigure}
     \caption{We analyze the performance of RFAC for different values of bandwidth b on HalfCheetah, Ant and Humanoid control tasks.
     While RFAC performs similarly on HalfCheetah and Ant for different values of bandwidth b, its performance varies on Humanoid with different values of b.}
     \label{fig:td3_rff_abl_bandwidth}
\end{figure}

==> figtext/rff_abl_f_dim.tex <==
\begin{figure}[t]
     \centering
     \includesvg[scale=0.3]{figures/ant_f_dim_4k_vs_400.svg}
     \caption{We analyze the performance of RFAC for state fourier dimensions on Ant. It suffers a significant drop in performance if we decrease its state fourier dimension from $4000$ to $400$.}
     \label{fig:td3_rff_abl_f_dim}
\end{figure}

==> figtext/rff_abl_indep_rff.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/HalfCheetah_conv.svg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/Ant_conv.svg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/Humanoid_conv.svg}
     \end{subfigure}
     \caption{RFAC's performance drops significantly on HalfCheetah, Ant, and Humanoid if we take Random Fourier Features independently per dimension via 1d convolution and then concatenate them.}
     \label{fig:td3_rff_indep_rff}
\end{figure}

==> figtext/rff_comp.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/HalfCheetah_comp.svg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/Ant_comp.svg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/Humanoid_comp.svg}
     \end{subfigure}
     \caption{We compare RFAC with \TD{} and other baselines on HalfCheetah, Ant and Humanoid control tasks. It improves over \TD{} and either matches or outperforms \TD-dense on all the tasks. \TD-deep improves over \TD{} and performs similar to RFAC and \TD-dense on HalfCheetah. On Ant and Humanoid, it performs similar to \TD{} implying that overparameterization doesn't always help.}
     \label{fig:td3_rff_comp}
\end{figure}

==> figtext/rff_dmc.tex <==
\begin{figure}[h]
     \centering
     \includesvg[scale=0.3]{figures/Hopper.svg}
     \caption{DeepMind Control suite domain: Hopper-hop. RFF network has lower variance, and out-performs the vanilla MLP baseline on average.}
     \label{fig:td3_rff_ant}
\end{figure}

==> figtext/rff_param_comp.tex <==
\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/HalfCheetah_comp_rff.svg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/Ant_comp_rff.svg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{figures/Humanoid_comp_rff.svg}
     \end{subfigure}
     \caption{We compare MLPs with different fourier feature parameterizations on how they perform on continous control tasks. We use \TD{} as the base reinforcement learning algorithm.
    %  We compare RFAC (i.e. \TD{}+RFN) with \TD{}+Siren and \TD{}+RFF-Tancik on HalfCheetah, Ant and Humanoid control tasks. We see that RFAC is able to outperform the other baselines which, in turn, shows that RFN is better suited for high dimensional continuous control tasks when compared to other random fourier feature paramterization.
     }
     \label{fig:rff_param_comp}
\end{figure}

==> figtext/td3_rff_ant.tex <==
\begin{figure}[h!]
     \centering
     \includesvg[scale=0.3]{figures/Ant_td3_rff.svg}
     \caption{RFF network applied to state-of-the-art TD3 algorithm on Ant. Showing significant performance gain, and a new state-of-the-art result.}
     \label{fig:td3_rff_ant}
\end{figure}

==> figtext/toy_mdp_decription.tex <==
\begin{figure}[t]
     \centering
     \includegraphics[width=\textwidth]{figures/toy_mdp_detail.pdf}
     \caption{Description of a toy MDP with $\gS = [0,1)$, $\gA = \{0,1\}$, $\gamma = 0.9$ and reward function $r(s,a)=s$. (a) describes its forward dynamics, (b) describes the ground truth Q function, (c) denotes the MLP fit to the Q function with fitted Q iteration (FQI)~\citep{fqi} after $200$ epochs and (d) denotes the same after $8000$ epochs.}
     \label{fig:toy_mdp_description}
\end{figure}
